XAI for Transformers: Better Explanations through Conservative Propagation

Transformers have become an important workhorse of machine learning, with numerous applications. This necessitates the development of reliable methods for increasing their transparency. Multiple interpretability methods, often based on gradient information, have been proposed. We show that the gradient in a Transformer reflects the function only locally, and thus fails to reliably identify the contribution of input features to the prediction. We identify Attention Heads and LayerNorm as main reasons for such unreliable explanations and propose a more stable way for propagation through these layers. Our proposal, which can be seen as a proper extension of the well-established LRP method to Transformers, is shown both theoretically and empirically to overcome the deficiency of a simple gradient-based approach, and achieves state-of-the-art explanation performance on a broad range of Transformer models and datasets.

==> Detaching LayerNorm and softmax for Transformer LRP /textparts.tex <==
% Previous IMDB table
\begin{table}[t]
\caption{Results for IMDB dataset.}
\label{tab:imdb}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc|ccr}
\hline
\abovespace\belowspace
Method      & AUAC & AUPC & Act-MSE  & Prune-MSE  \\
\hline
\abovespace
Random       & 0.679 &  0.682 &  2.041 & 2.028\\
A-Last       & 0.714 &  0.705 &  1.543 &  1.646  \\
A-Flow       & -     & - &  -     & -\\
Saliency     & 0.820 & 0.742 &  2.281 & 1.032 \\
Rollout      & 0.746 &  0.738 &  0.902  &  1.017 \\
GI           & 0.922 & 0.744 &  2.717   & 0.849 \\
LRP          & 0.907 & 0.741 &  2.353  & 0.902 \\
\hline
GI  D-LN-SM  & \textbf{0.942} & \textbf{0.755} &  \textbf{3.692} & \textbf{0.643}\\
LRP D-LN-SM  & \textbf{0.941} & \textbf{0.754} &  3.560& 0.657 \\

\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}



%


\begin{table}[t]
\caption{Results for BBBP dataset.}
\label{bbbp}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\hline
\abovespace\belowspace
Method & Rec-AUC & Diff-AUC & Fidelity AUC  \\
\hline
\abovespace
Random       &  &  &   \\
A-Last       &  &  &     \\
A-Flow       &  &  &    \\
Saliency     &  &  &    \\
Rollout      & &  &    \\
LRP          &  &  &     \\
\hline
LRP D-LN-SM  &  &  &    \\
LRP D-SM     &  &  &    \\

\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}



% Old sst


\begin{table}[t]
\caption{Results for SST2 dataset.}
\label{sst}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\hline
\abovespace\belowspace
Method & Rec-MSE & Prune-MSE & AUAC  \\
\hline
\abovespace
Random       & 3.817 & 4.101 & 0.663  \\
A-Last       & 2.317 & 2.567 & 0.709    \\
A-Flow       & 2.318 & 2.581 & 0.708   \\
Saliency     & \textbf{2.249} & 2.188 & 0.770   \\
Rollout      & 2.286 & 2.581 & 0.708   \\
LRP          & 3.054 & 2.034 & 0.847    \\
\hline
LRP D-LN-SM  & 3.442 & \textbf{1.543} & \textbf{0.908}   \\
LRP D-SM     & 3.190 & \textbf{1.801} & 0.855   \\

\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> textparts.tex <==
% Previous IMDB table
\begin{table}[t]
\caption{Results for IMDB dataset.}
\label{tab:imdb}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc|ccr}
\hline
\abovespace\belowspace
Method      & AUAC & AUPC & Act-MSE  & Prune-MSE  \\
\hline
\abovespace
Random       & 0.679 &  0.682 &  2.041 & 2.028\\
A-Last       & 0.714 &  0.705 &  1.543 &  1.646  \\
A-Flow       & -     & - &  -     & -\\
Saliency     & 0.820 & 0.742 &  2.281 & 1.032 \\
Rollout      & 0.746 &  0.738 &  0.902  &  1.017 \\
GI           & 0.922 & 0.744 &  2.717   & 0.849 \\
LRP          & 0.907 & 0.741 &  2.353  & 0.902 \\
\hline
GI  D-LN-SM  & \textbf{0.942} & \textbf{0.755} &  \textbf{3.692} & \textbf{0.643}\\
LRP D-LN-SM  & \textbf{0.941} & \textbf{0.754} &  3.560& 0.657 \\

\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}



%


\begin{table}[t]
\caption{Results for BBBP dataset.}
\label{bbbp}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\hline
\abovespace\belowspace
Method & Rec-AUC & Diff-AUC & Fidelity AUC  \\
\hline
\abovespace
Random       &  &  &   \\
A-Last       &  &  &     \\
A-Flow       &  &  &    \\
Saliency     &  &  &    \\
Rollout      & &  &    \\
LRP          &  &  &     \\
\hline
LRP D-LN-SM  &  &  &    \\
LRP D-SM     &  &  &    \\

\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}



% Old sst


\begin{table}[t]
\caption{Results for SST2 dataset.}
\label{sst}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\hline
\abovespace\belowspace
Method & Rec-MSE & Prune-MSE & AUAC  \\
\hline
\abovespace
Random       & 3.817 & 4.101 & 0.663  \\
A-Last       & 2.317 & 2.567 & 0.709    \\
A-Flow       & 2.318 & 2.581 & 0.708   \\
Saliency     & \textbf{2.249} & 2.188 & 0.770   \\
Rollout      & 2.286 & 2.581 & 0.708   \\
LRP          & 3.054 & 2.034 & 0.847    \\
\hline
LRP D-LN-SM  & 3.442 & \textbf{1.543} & \textbf{0.908}   \\
LRP D-SM     & 3.190 & \textbf{1.801} & 0.855   \\

\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

